Introduction to the Special Issue on Sounding Rockets and Instrumentation

Rocket technology, originally developed for military applications, has provided a low-cost observing platform to carry critical and rapid-response scientific investigations for over 70 years. Even with the development of launch vehicles that could put satellites into orbit, high altitude sounding rockets have remained relevant. In addition to science observations, sounding rockets provide a unique technology test platform and a valuable training ground for scientists and engineers. Most importantly, sounding rockets remain the only way to explore the tenuous regions of the Earth's atmosphere (the upper stratosphere, mesosphere, and lower ionosphere/thermosphere) above balloon altitudes ($\sim$40 km) and below satellite orbits ($\sim$160 km). They can lift remote sensing telescope payloads with masses up to 400 kg to altitudes of 350 km providing observing times of up to 6 minutes above the blocking influence of Earth's atmosphere. Though a number of sounding rocket research programs exist around the world, this article focuses on the NASA Sounding Rocket Program, and particularly on the astrophysical and solar sounding rocket payloads.

==> sec-conclusion.tex <==
% !TEX root = JAI2015-intro.tex

Sounding rockets guided science into the Space Age. Where once they were the pinnacle of technological achievement, they are still the guides on the frontier, testing technologies, science, and people for bigger things.
